Entanglement Increases the Error-Correcting Ability of Quantum Error-Correcting Codes

If entanglement is available, the error-correcting ability of quantum codes can be increased. We show how to optimize the minimum distance of an entanglement-assisted quantum error-correcting (EAQEC) code, obtained by adding ebits to a standard quantum error-correcting code, over different encoding operators. By this encoding optimization procedure, we found several new EAQEC codes, including a family of [[n, 1, n; n-1]] EAQEC codes for n odd and code parameters [[7, 1, 5; 2]], [[7, 1, 5; 3]], [[9, 1, 7; 4]], [[9, 1, 7; 5]], which saturate the quantum singleton bound for EAQEC codes. A random search algorithm for the encoding optimization procedure is also proposed.

==> AlgorithmImprovement.tex <==
%%%% Examples
%%%%

\be Table \ref{tb:7BCHcode} provides the parameters that can be
obtained if a standard $[[7,1,3]]$ quantum BCH
code\cite{gb99,AKS05} is optimized.
%the encoding optimization algorithm is applied on
%\begin{table}[bht]
%  \centering
%  \caption{Optimization over a $[[7,1,3]]$ Quantum BCH code} \label{tb:7BCHcode}
%  \begin{tabular}{|c|cccccc|}
%\hline
%      $c$& $6$& $5$& $4$& $3$& $2$&  $1$\\
%\hline
%      $d$& $7$& $5$& $5$& $5$& $5$&  $3$\\
%\hline
% \end{tabular}
%\end{table}
\begin{table}[bht]
  \centering
  \caption{Best minimum distance achieved and the average number of trials in the random search algorithm for optimizing the $[[7,1,3]]$ quantum BCH code} \label{tb:7BCHcode}
  \begin{tabular}{|c|c|c|c|c|c|}
\hline
      $c$&    $d_e$& $d_s$ & $N_{max}$& $2^{2ck}N(r,c)$  & $2^{2ck}N(r,c)/N_{max}$\\
      \hline
6 &  7 & 5 &36  &4096&    113.78\\
5 &  5 & 5 &31920  & 64512 &  2.02\\
4 &  5 & 5 &39522  & 166656 & 4.22\\
3 &  5 & 4 &4332   &89280 &  20.61\\
2 &  5 & 3 &14  &10416 &  744 \\
1 &  3 & 3 &252&  252&  1\\
\hline
 \end{tabular}
\end{table}
%$[[7,1,7;6]]$, $[[7,1,5;5]]$, $[[7,1,5;4]]$, $[[7,1,5;3]]$, $[[7,1,4;2]]$, and $[[7,1,3;1]]$.
%\[[[7,1,7;6]],\] \[[[7,1,5;5]],\] \[[[7,1,5;4]],\] \[[[7,1,5;3]],\] \[[[7,1,4;2]],\] and \[[[7,1,3;1]].\]
Note that the parameters $[[7,1,7;6]]$, $[[7,1,5;3]]$ and
$[[7,1,5;2]]$ achieve the quantum singleton bound for EAQECC
(\ref{eq:singleton_bound}) and are not equivalent to any standard
quantum stabilizer codes. In addition, we compare the
$[[7,1,5;3]]$ EAQEC code by the encoding optimization to a
competing EAQEC code with $n=7$ and $d=5$ by the construction of
\cite{BDM06} or the binary version (\ref{eq:construction Brun}).
According to Grassl's table at \cite{Grassl}, a classical linear
code over $GF(4)$ (or $GF(2)$) that meets our requirement is a
$[7,2,5]$ linear quartenary code, which can be utilized to
contruct a $[[7,2,5; 5]]$ EAQEC code.
%$[[7,c-3,5; c]]$ EAQEC code for a certain $c$.
It can be observed that the $[[7,1,5;3]]$ EAQEC code cannot be
obtained by the construction of \cite{BDM06} with $c=3$.
Therefore, the $[[7,1,5;3]]$ EAQEC code is new. \eep


\be We apply the random search algorithm for encoding optimization
on the $[[7,1,3]]$ quantum BCH code,  Shor's $[[9,1,3]]$
code\cite{Shor95}, and the $[[13,1,5]]$ quantum QR
code\cite{CRSS97,LLu07} $1000$ times for each $c$ and the results
are shown in Table \ref{tb:7BCHcode}, \ref{tb:9BCHcode}, and
\ref{tb:13BCHcode}. As shown in these tables, $d_e$ is the minimum
distance of the EAQEC codes we find in the random search algorithm
and $d_s$ is the best minimum distance for an $[[n+c,1,d_s]]$
standard quantum code in Grassel's table\cite{Grassl}. The merit
functions we adopted are $m_1(f(x))= \sum_{i=1}^n a_i\cdot i$ and
$m_2(f(x))= \sum_{i=1}^b a_i\cdot i$, where $b=\lfloor
\frac{n-k+c+2}{2}\rfloor$ from the quantum singleton bound.
%We perform the random search algorithm and the average number of trials to achieve to the minimum distance we obtained are shown in these tables.
It seems intuitively that the weights that really matter are those
below the quantum singleton bound. However, the average numbers of
trials needed for these two merit functions are very close, and
the average number of trial is relatively low compared with
$2^{2ck}N(r,c)$ for a complete encoding optimization in each case.
For the $[[7,1,3]]$ quantum BCH code, the random search algorithm
achieves the same result as a complete encoding optimization. The
minimum distances of the EAQEC codes found from the random search
algorithm on the $[[9,1,3]]$, $[[13,1,5]]$ codes are also better
than or equal to that of the corresponding standard
$[[n+c,k,d_s]]$ codes. Therefore, the random search algorithm for
encoding optimization seems to be an efficient method to partially
optimize an encoding operator.

%\begin{table}[bht]
%  \centering
%  \caption{Best minimum distance achieved and the average number of trials in the random search algorithm for optimizing the $[[7,1,3]]$ quantum BCH code} \label{tb:7BCHcode}
%  \begin{tabular}{|c|c|c|c|c|c|}
%\hline
%      $c$&    $6$& $5$& $4$& $3$& $2$\\
%      \hline
%      $d$&    $7$& $5$& $5$& $5$& $5$\\
%      \hline
%      $d'$&    $5$& $5$& $5$& $4$&\\
%      \hline
%      fully random &  $120.46$ & $2.80$ & $13.56$ & $552.624$& \\
%%      one bit random&
%      $m_2$& $112.4$ & $8.18$ & $70.17$ & $10021.08$&\\
%     $2^{2rk}N(r,c)$ & $4096$ & $64512$& $166656$& $89280$& $10416$\\
%     max & $36$ & $31920$ & $127134$ & $4332$& $14$\\
%\hline
% \end{tabular}
%\end{table}
\begin{table}[bht]
  \centering
  \caption{Best minimum distance achieved and the average number of trials in the random search algorithm for optimizing Shor's $[[9,1,3]]$  code} \label{tb:9BCHcode}
  \begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
      $c$&    $8$& $7$& $6$& $5$ & $4$ & $3$ &2 \\
      \hline
      $d$&    $9$& $7$& $7$& $7$ &$7$& $5$&$5$\\
      \hline
      $d'$&    $7$& $6$& $5$& $5$&&\\
      \hline
      random & $ $ & $ $ &$ $ &$ $&&\\
       &   & $ $ &$ $ &$ $&&\\
       $N_C=d_{max}$ & $256$ &  $330624$ & $278904$ &$17748 $& $132$& $69777$ & $201$\\
      $2^{2ck}N(r,c)$ & $65536$ & $4.17\times 10^{6}$& $4.42\times 10^{7}$& $9.94\times 10^{7}$& $5.14\times 10^7$& $6.21\times 10^6$ & $1.72\times 10^5$ \\
\hline
 \end{tabular}
\end{table}
\begin{table}[bht]
  \centering
  \caption{Best minimum distance achieved and the average number of trials in the random search algorithm for optimizing the $[[13,1,5]]$ quantum QR code} \label{tb:13BCHcode}
  \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
      $c$&    $12$& $11$& $10$& $9$ & $8$& $7$\\ %& $6$\\
      \hline
      $d$&    $13$& $11$& $11$& $9$ & $9$& $7$\\ %& $7$\\
       \hline
      $d'$&    $9$& $8-9$& $7-9$& $7-8$ & $7$& $7$\\ %& $7$\\
      \hline
      $m_1$& $33609.24$ & $3216.50$ & $19.61$ & $983.43$ & $4269.63$ & $9.48$ \\ %&$90.208$\\
      $m_2$& $32589.23$ &$3265.54$&$18.28$&$1046.47$&$4042.06$ &$8.76$\\ % &$94.561$\\
      $2^{2ck}N(r,c)$ & $1.67\times 10^{7}$ & $1.71\times 10^{10}$&$2.92\times 10^{12 }$ & $1.07\times 10^{15 }$ &$9.11\times 10^{15 }$& $1.87\times 10^{16}$\\
       $number$&    $456$& $ $& $ $& $ $ & $ $& $ $\\ %& $7$\\
\hline
 \end{tabular}
  \begin{tabular}{|c|c|c|c|c|c|c|}
\hline
      $c$&    $6$& $5$& $4$&  &&\\ %& $6$\\
      \hline
      $d$&    $7$& $7$& $7$\\
       \hline
      $d'$&    $9$& $8-9$& $7-9$& $7-8$ & $7$& $7$\\ %& $7$\\
      \hline
      $m_1$&\\
      $m_2$&\\
      $2^{2ck}N(r,c)$ &  & $1.17\times 10^{14}$&$3.56\times 10^{12 }$\\
       $number$&    & $ $& $ $& $ $ & $ $& $ $\\ %& $7$\\
\hline
 \end{tabular}
\end{table}
























%\subsection{Further Improvement on the Encoding Optimization} \label{Sec:Improvement}
%In this section,
%Next, we show that effects of the operator $W$ and $V$ can be combined. %to simplify and this may reduce the complexity of the encoding optimization algorithm.
%We illustrate the idea with an example.


%
%
%$[[7,1,3]]$ quantum BCH code is
%\[
%H_0=\begin{bmatrix}
%0000000 & 1001011\\
%0000000 & 0101110\\
%0000000 & 0010111\\
%1001011 & 0000000\\
%1100101 & 0000000\\
%1011100 & 0000000\\
%\end{bmatrix}.
%\]
%Applying Wilde's algorithm, we can obtain an encoding operator $U_E$.
%The $[[ 7,1,5;3]]$ EAQEC code in Table \ref{tb:7BCHcode} is obtained by applying encoding optimization with
%\[
%A=\begin{bmatrix}
%101000
%\end{bmatrix}^T,
%\
%B=\begin{bmatrix}
%100000
%\end{bmatrix}^T,
%\]
%and
%\[
%G_{3\times 6}=
%\begin{bmatrix}
%100110\\
%010101\\
%001010
%\end{bmatrix},
%\]
%and it has a check matrix
%$
%\begin{bmatrix}
%G'_{3\times 6}H_0\\
%\hline
%0101000 \ 0100010\\
%1001000 \ 0010010\\
%0100100 \ 0000011\\
%\end{bmatrix},
%$
%where
%$
%G'_{3\times 6}=
%\begin{bmatrix}
%100000\\
%010000\\
%001000\\
%110100\\
%101010\\
%010001
%\end{bmatrix}.
%$
%Note that the symplectic relations hold in the above matrix.
%The initial state $\ket{\psi}=\ket{000000}\ket{\phi}$ has a logical $Z$ operator $Z_7$ and a logical $X$ operator $X_7$.
 %For convenience, if $U$ is a unitary operator, we define a homomorphism $\lambda_U$ on a Pauli matrix $M$ by
%\[
%\lambda_U(M)= UMU^{\dag}.
%\]
%From the matrices $A$ and $B$, we have
%\[
%\lambda_W(X_1)=X_1X_7Z_7,
%\]
%\[
%\lambda_W(X_3)=X_3X_7,
%\]
%and
%\[
%\lambda_W(X_i)=X_i,
%\]
%for $i=2,4,5,6$.
%From the matrix $G_{3\times 6}$, we have
%\[
%\lambda_{VU_EW}(X_1)=\lambda_{U_EW}(X_1)\lambda_{U_EW}(X_4)\lambda_{U_EW}(X_5)=\lambda_{U_E}(X_1X_4X_5X_7Z_7),
%\]
%\[
%\lambda_{VU_EW}(X_2)=\lambda_{U_EW}(X_2)\lambda_{U_EW}(X_4)\lambda_{U_EW}(X_6)=\lambda_{U_E}(X_2X_4X_6),
%\]
%and
%\[
%\lambda_{VU_EW}(X_3)=\lambda_{U_EW}(X_3)\lambda_{U_EW}(X_5)=\lambda_{U_E}(X_3X_5X_7).
%\]
%In general, we have $\lambda_{VU_E}(X_i)=\lambda_{U_EV}(X_i)$  and $\lambda_{VU_E}(Z_j)=\lambda_{U_EV}(Z_j)$.
%Thus \[\lambda_{VU_E W}(X_i)=\lambda_{U_E VW}(X_i)=\lambda_{U_E}(\lambda_{VW}(X_i)).\]
%%Similarly,  \[\lambda_{VU_E W}(Z_j)=\lambda_{U_E VW}(Z_j)=\lambda_{U_E}(\lambda_{VW}(Z_j)).\]
%It can be observed that the three additional stabilizer
%generators are obtained by applying the encoding operator $U_E$ on
%Pauli operators of the form
%\[
% X_1^{d_1}X_2^{d_2} X_3^{d_3} X_4^{d_4} X_5^{d_5} X_6^{d_6} X_7^{d_7}Z_7^{d_8},
%\]
%where $d_i$'s $\in\{0,1\}$ and $\sum_{i=1}^{6} d_i >0$.
%Consequently, if we want to add $c$ ebits to an $[[n,k]]$ standard code to increase the minimum distance of the code,
%it suffices to choose $c$ linearly independent operators from fewer than $2^{n+k}$ operators
%\[
%X_1^{d_1}\cdots X_n^{d_n} Z_{r+1}^{d_{n+1}}\cdots Z_{r+k}^{d_{n+k}} ,
%\]
%where $d_i$'s $\in\{0,1\}$ and $\sum_{i=1}^{r} d_i >0$.
%To determine the number of possible choices is
%Similar to the number of possible matrices $G_{c\times r}$ (\ref{eq:number of row operations}) in encoding optimization,
%the number of possible choices is \[2^{2ck}N(r,c),\]% with $r$ replaced by $n+k$.
%\begin{align} \label{eq:number of optimization}
%2^{2ck}\sum_{i_c=0}^{r-c}
%\sum_{i_{c-1}=0}^{r-c-i_c}\sum_{i_{c-2}}^{r-c-i_{c}-i_{c-1}}\cdots
%\sum_{i_1=0}^{r-c-\sum_{j=1}^c i_j}  2^{ c(r-c-\sum_{l=1}^c i_l)
%+\sum_{m=1}^{c-1} i_m(c-m)}.
%\end{align}
%There are fewer than
%which is bounded by
%, where $W$ commutes with $Z_i$'s   %that leaves $Z_1$, $\cdots$, $Z_r$ invariant
%and $V$ is a row operation, optimized over  %\begin{align*}
%\[{r\choose c} \cdot 2^{c(n+k-c)}.\]
%possibilities.
%Although this upper bound is better than (\ref{bound:row_operation_selecting_operation}), it grows exponentially as $n+k$ increases.


==> BasicEAQEC.tex <==


\section{Basic of EAQEC} \label{Sec:BasicEAQEC}

For a $n-$qubit initial state $\ket{\psi}$ with $k$ qubits information and $r=n-k$ ancilla qubits,
\[\ket{\psi}=\ket{00\cdots0}\ket{\phi_1}\cdots\ket{\phi_k},\]
its stabilizer group has generators
\[
Z_1, Z_2, \cdots, Z_r
\]
and logical operators
\[
Z_{r+1}, \cdots, Z_{n},
\]
\[
X_{r+1}, \cdots, X_{n},
\]
Suppose we have an encoding operator $U$. Then the stabilizer group $\mathcal{S}$ of the encoded state $U\ket{\psi}$ is generated by
\[
g_1= UZ_1U^{\dag}, \cdots, g_r= UZ_rU^{\dag}
\]
and the logical operators are
\[
l_1= UZ_{r+1}U^{\dag}, \cdots, l_k= UZ_{n}U^{\dag},
\]
\[
m_1= UX_{r+1}U^{\dag}, \cdots, m_k= UX_nU^{\dag}.
\]
Note that the logical operators commute with the stabilizers.
Hence the normalizer group of $\mathcal{S}$ is
\[
N(\mathcal{S})= \langle g_1,g_2,\cdots, g_r, l_1,l_2,\cdots, l_k, m_1,m_2,\cdots, m_k  \rangle
\]
with dimension $2n-r=r+2k.$
The minimum distance of the stabilizer code defined by $\mathcal{S}$  is the minimum weight of an element in
\[
N(\mathcal{S})-\mathcal{S}=  \langle g_1,g_2,\cdots, g_r, l_1,l_2,\cdots, l_k, m_1,m_2,\cdots, m_k  \rangle-  \langle g_1,g_2,\cdots, g_r\rangle.
\]


For a $n-$qubit initial state $\ket{\psi}$ with $k$ qubits information, $c$ pairs of maximally-entangled states and $n-k-c=r-c$ ancilla qubits,
\[\ket{\psi}=\ket{\Phi_+}^{AB}\cdots \ket{\Phi_+}^{AB}\ket{00\cdots0}\ket{\phi_1}\cdots\ket{\phi_k},\]
its stabilizer group has generators
\[
Z_1, Z_2, \cdots, Z_c, Z_{c+1},\cdots, Z_{r}
\]
\[
X_1, X_2, \cdots, Z_c,
\]
and logical operators
\[
Z_{r+1}, \cdots, Z_{n},
\]
\[
X_{r+1}, \cdots, X_{n},
\]
Suppose we have an encoding operator $U$. Then the simplified stabilizer group $\mathcal{S}$ of the encoded state $U\ket{\psi}$ is generated by
\[
g_1= UZ_1U^{\dag}, \cdots, g_r= UZ_rU^{\dag},
\]
\[
h_1= UX_1U^{\dag}, \cdots, h_c= UX_cU^{\dag}
\]
and the logical operators are
\[
l_1= UZ_{r+1}U^{\dag}, \cdots, l_k= UZ_{n}U^{\dag},
\]
\[
m_1= UX_{r+1}U^{\dag}, \cdots, m_k= UX_nU^{\dag}.
\]
The symplectic subgroup $\mathcal{S}_S=\langle g_1,\cdots, g_c, h_1,\cdots,h_c  \rangle.$
The isotropic subgroup $\mathcal{S}_I=\langle g_{c+1},\cdots, g_r \rangle.$
Note that the logical operators commute with the stabilizers.
Hence the normalizer group of $\mathcal{S}$ is
\[
N(\mathcal{S})= \langle g_{c+1},\cdots, g_r, l_1,l_2,\cdots, l_k, m_1,m_2,\cdots, m_k  \rangle
\]
with dimension $2n-r-c=2k+r-c.$
The minimum distance of the stabilizer code defined by $\mathcal{S}$  is the minimum weight of an element in
\[
N(\mathcal{S})-\mathcal{S}_I=  \langle g_{c+1},\cdots, g_r, l_1,l_2,\cdots, l_k, m_1,m_2,\cdots, m_k  \rangle-  \langle g_{c+1},\cdots, g_r\rangle.
\]
In the case $c=r$, we have $\mathcal{S}_S=\mathcal{S}$, $\mathcal{S}_I=\varnothing$ and
\[
N(\mathcal{S})= \langle l_1,l_2,\cdots, l_k, m_1,m_2,\cdots, m_k  \rangle
\]
with dimension $2n-2r=2k.$
The minimum distance of the stabilizer code defined by $\mathcal{S}$  is the minimum weight of an element in
\[
N(\mathcal{S})=  \langle l_1,l_2,\cdots, l_k, m_1,m_2,\cdots, m_k  \rangle.
\]

